Hallucination is Inevitable: An Innate Limitation of Large Language Models

Hallucination has been widely recognized to be a significant drawback for large language models (LLMs). There have been many works that attempt to reduce the extent of hallucination. These efforts have mostly been empirical so far, which cannot answer the fundamental question whether it can be completely eliminated. In this paper, we formalize the problem and show that it is impossible to eliminate hallucination in LLMs. Specifically, we define a formal world where hallucination is defined as inconsistencies between a computable LLM and a computable ground truth function. By employing results from learning theory, we show that LLMs cannot learn all the computable functions and will therefore inevitably hallucinate if used as general problem solvers. Since the formal world is a part of the real world which is much more complicated, hallucinations are also inevitable for real world LLMs. Furthermore, for real world LLMs constrained by provable time complexity, we describe the hallucination-prone tasks and empirically validate our claims. Finally, using the formal world framework, we discuss the possible mechanisms and efficacies of existing hallucination mitigators as well as the practical implications on the safe deployment of LLMs.

==> sec_hallucination_prone_problems.tex <==
\section{Details of Identified Hallucination-prone Problems}\label{sec:details_hallcunation_prone_problems}

\subsection{Description of Hallucination-Prone Problems}

\begin{table*}[ht!]
    \centering
    \caption{Identified hallucination-prone problems. This is a copy of \cref{tab:hallucination_prone_problems_all}.}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}llll@{}}
        \toprule
        LLMs                                                                                                          & Problem                                                                   & Hallucination Guaranteed by                                            & Extra Assumption             \\ \midrule
        \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}$P$-proved $O(n^k)$ LLMs\\ (incl. all existing LLMs)\end{tabular}} & Combinatorial List                                                        & Requiring $O(2^{n})$ solution                                          & None                         \\ \cmidrule(l){2-4} 
                                                                                                                      & Subset Sum                                                                & Being NP-complete                                                      & $\text{P} \neq \text{NP}$    \\ \cmidrule(l){2-4} 
                                                                                                                      & Boolean Satisfiability (SAT)                                              & \begin{tabular}[c]{@{}l@{}} Being NP-complete \\ \cite{Cook1971ComplexityTPP} \end{tabular}                         & $\text{P} \neq \text{NP}$    \\ \cmidrule(l){2-4} 
                                                                                                                      & Entailment of Propositional Logic                                         & \begin{tabular}[c]{@{}l@{}} Being co-NP-complete\\ \cite{Arora2009ComputationalCAMA} \end{tabular}  & $\text{P} \neq \text{co-NP}$ \\ \midrule
        \begin{tabular}[c]{@{}l@{}}$P$-proved $O(2^n)$ LLMs,\\ $P$-proved $O(n^k)$ LLMs\end{tabular}                  & \begin{tabular}[c]{@{}l@{}} Presburger Arithmetic \\ \cite{Presburger1929UberDV,Stansifer1984presburger} \end{tabular} & \begin{tabular}[c]{@{}l@{}} Requiring $O(2^{2^{n}})$ solution\\ \cite{Fischer1998SuperexponentialCO} \end{tabular} & None                         \\ \midrule
        \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}All Computable LLMs\\ (incl. all LLMs above)\end{tabular}}         & Learning all Computable Linear Orders                                     & \cref{thm:hallucination_linear_order}                                  & None                         \\ \cmidrule(l){2-4} 
                                                                                                                      & Solving all Computable Problems                                           & \cref{thm:llm_fails_computable}                                        & None                         \\ \cmidrule(l){2-4} 
                                                                                                                      & Entailment of First-Order Logic                                           & \begin{tabular}[c]{@{}l@{}} Being Undecidable \\ \cite{Turing1936ComputableNW} \end{tabular}                        & None                         \\ \bottomrule
        \end{tabular}%
        }
\end{table*}

For ease of reference, we copy \cref{tab:hallucination_prone_problems_all} here.
In each problem listed in the table, ground truth $f$ is expected to have the following behavior:

\begin{itemize}
	\item\label{enu:list_exp} Combinatorial List: $f$ lists all the strings with length $m$ using an alphabet of two characters. Computing $f$ takes $O(2^{m})$ time.
	\item Presburger arithmetic~\cite{Presburger1929UberDV,Stansifer1984presburger}: Presburger arithmetic is the first-order theory of natural numbers with addition and order $<$. Given a statement in the arithmetic, $f$ returns ``yes'' if the statement can be proved within the arithmetic and ``no'' otherwise. Computing $f$ takes $O(2^{2^{\Pi(m)}})$ time~\cite{Fischer1998SuperexponentialCO}. 
	\item\label{item:subsetsum} Subset Sum: given a set of $m$ integers and a number $q$, $f$ returns ``yes'' when there is a subset that sums up to $q$ and ``no'' otherwise. This problem is NP-complete.
	\item\label{item:sat} Boolean Satisfiability (SAT)~\cite{Cook1971ComplexityTPP}: given a formula of $m$ Boolean variables, $f$ returns ``yes'' if there exists an assignment on these variables which results in the formula to be true and ``no'' otherwise. This problem is NP-complete~\cite{Cook1971ComplexityTPP}.
	\item\label{item:entail} Entailment of propositional logic: given two propositional logic formulas $\psi$ and $\phi$, let $M(\psi)$ be the set of all the models of $\psi$, $f$ returns ``yes'' if $M(\psi) \subseteq M(\phi)$ and ``no'' otherwise. This problem is co-NP-complete~\cite{Arora2009ComputationalCAMA}.
	\item \label{item:entail_fol} Entailment of first-order logic: given two first-order logic formulas $\psi$ and $\phi$, let $M(\psi)$ be the set of all the models of $\psi$, $f$ returns ``yes'' if $M(\psi) \subseteq M(\phi)$ and ``no'' otherwise. This problem is undecidable~\cite{Turing1936ComputableNW}.
\end{itemize}

As a result, real-world LLMs' answers about mathematical problems and logic reasoning should always be subject to proper scrutiny.
The result is supported by a recent study~\cite{Hong2024stuckQN}.
In \cref{sec:empirical_list_exponential}, we provide an empirical study to illustrate the combinatorial list problem.
In \cref{ssec:linear_order}, we detail the problem of learning all computable linear orders and provide empirical results.

